Mode Recognition by Shape Morphing for Maxwell's Eigenvalue Problem

In electrical engineering, for example during the design of superconducting radio-frequency cavities, eigenmodes must be identified based on their field patterns. This allows to understand the working principle, optimize the performance of a device and distinguish desired from parasitic modes. For cavities with simple shapes, the eigenmodes are easily classified according to the number of nodes and antinodes in each direction as is obvious from analytical formulae. For cavities with complicated shapes, the eigenmodes are determined numerically. Thereby, the classification is cumbersome, if not impossible. In this paper, we propose a new recognition method by morphing the cavity geometry to a pillbox and tracking its eigenmodes during the deformation.

==> 9cellMorphing.tex <==
\begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth, trim =30mm 68mm 30mm 68mm, clip]{figures/efield_mode9/efield_mode9_wBP_ttf.0000.jpeg}
  \caption{Magnitude of the electric field at $t = 0.00$.}
  \label{fig:0000}
 \end{subfigure}
 \begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth, trim =30mm 68mm 30mm 68mm, clip]{figures/efield_mode9/efield_mode9_wBP_ttf.0003.jpeg}
  \caption{Magnitude of the electric field at $t = 0.15$.}
  \label{fig:0003}
 \end{subfigure}
 \begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth, trim =30mm 68mm 30mm 68mm, clip]{figures/efield_mode9/efield_mode9_wBP_ttf.0012.jpeg}
  \caption{Magnitude of the electric field at $t = 0.60$.}
  \label{fig:0012}
 \end{subfigure}
  \begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth, trim =30mm 68mm 30mm 68mm, clip]{figures/efield_mode9/efield_mode9_wBP_ttf.0016.jpeg}
  \caption{Magnitude of the electric field at $t = 0.80$.}
  \label{fig:0016}
 \end{subfigure}
 \begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth, trim =30mm 68mm 30mm 68mm, clip]{figures/efield_mode9/efield_mode9_wBP_ttf.0019.jpeg}
  \caption{Magnitude of the electric field at $t = 0.95$.}
  \label{fig:0019}
 \end{subfigure}
 \begin{subfigure}[b]{1.0\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth, trim =30mm 68mm 30mm 68mm, clip]{figures/efield_mode9/efield_mode9_wBP_ttf.0020.jpeg}
  \caption{Magnitude of the electric field at $t = 1.00$.}
  \label{fig:0020}
 \end{subfigure}
